No-Regret Learning in Dynamic Stackelberg Games

In a Stackelberg game, a leader commits to a randomized strategy, and a follower chooses their best strategy in response. We consider an extension of a standard Stackelberg game, called a discrete-time dynamic Stackelberg game, that has an underlying state space that affects the leader's rewards and available strategies and evolves in a Markovian manner depending on both the leader and follower's selected strategies. Although standard Stackelberg games have been utilized to improve scheduling in security domains, their deployment is often limited by requiring complete information of the follower's utility function. In contrast, we consider scenarios where the follower's utility function is unknown to the leader; however, it can be linearly parameterized. Our objective then is to provide an algorithm that prescribes a randomized strategy to the leader at each step of the game based on observations of how the follower responded in previous steps. We design a no-regret learning algorithm that, with high probability, achieves a regret bound (when compared to the best policy in hindsight) which is sublinear in the number of time steps; the degree of sublinearity depends on the number of features representing the follower's utility function. The regret of the proposed learning algorithm is independent of the size of the state space and polynomial in the rest of the parameters of the game. We show that the proposed learning algorithm outperforms existing model-free reinforcement learning approaches.

==> tex/online_learning_theta_old.tex <==

\subsection{Online learning $\theta^*$}

Let $A = \{a_1, ..., a_n\}$ and $B=\{b_1, ..., b_m\}$.
In this section, we assume that the follower's reward function is linearly parameterized. That is, there exists a feature mapping $f : A \times B \to \R^p$ 
\begin{equation}
    r^1(a,b) = \langle f(a,b) , \theta^* \rangle
\end{equation}
for some $\theta* \in \R^p$. For ease of notation, we define the following matrices, called \emph{feature matrices}, for each action $b \in B$. $M_b \in \R^{n \times p}$ such that
\begin{equation}
    [M_b]_{ij} = [f(a_i,b)]_j.
\end{equation}
\begin{equation}
    [M_b]_{i} = [f(a_i,b)].
\end{equation}
Let $\varphi : A \to B$ represent the follower agent's optimal policy
\begin{equation}
    \varphi(a) = \argmax_{b \in B} r^1(a,b).
\end{equation}
We also define reward vectors $R^0_{s,b} \in \R^n$
\begin{equation}
    [R^0_{s,b}]_i = r^0(s,a_i,b).
\end{equation}
Let $\Pi$ be the set of mixed policies $S \to \Delta(A)$.
We aim to minimize the regret
  \begin{align}
    \regret(T) = \sup_{\pi \in \Pi} \E[ \sum_{t=1}^T r^0(s_t^{\pi}, a_t^{\pi}, \varphi(a^{\pi}_t) ) ]
    - \E [ \sum_{t=1}^T r^0(a_t, s_t, \varphi(a_t)) ]
    \label{def:regret}
  \end{align}
 We define the instantaneous value and action-value function with respect to policy $\pi$ and episode $t$ as
 \begin{align}
     Q^{\pi}(s,a) &= \E_{\pi} \left[\sum_{t=1}^{T} r^0(s_t, a_t, \varphi(a_t)) \mid s_1 = s, a_1 = a \right], \\
      V^{\pi}(s) &= \sum_{a} \pi(a|s) Q^{\pi}(s,a)
 \end{align}
 where the states $s_k$ and action $a_k$ are taken in expectation over $\pi$.
 We can also define the \emph{average reward per stage} for $\pi$:
 \begin{align}
     \rho^{\pi} &= \lim_{T \to \inf} \frac{1}{T} \sum_{t=1}^T \E_{\pi} \left[ r^0(s_t, a_t, \varphi(a_t)) \right] \\
                &= \sum_{s} \mu^{\pi}(s)\sum_{a}\pi(a|x) r^0(s,a,\varphi(a))
 \end{align}
 where $\mu^{\pi}$ is the stationary distribution underlying $\pi$. \fromnik{Do we need to use the concept of average reward?}
 With these definitions, we can relate the regret beginning in state $s_1$ to 
 \begin{equation}
     \regret(T) = \sup_{\pi} \sum_{t=1}^T (V^{\pi}(s_1) - V^{\pi_t}(s_1))
 \end{equation}
 where $\pi_t$ is the policy chosen by the learner at stage $t$.

Therefore, whenever we receive a sample $(X, b)$, we know that $\forall b' \in B$
\begin{align}
    \E_{a \samp X} [r^1(a, b)] & \geq  \E_{a \samp X} [r^1(a, a)] {\color{red}{\text{ Abolfazl: }r^1(a, b')?}} \\
    \E_{a \samp X} [\langle f(a, b), \theta \rangle] &\geq  \E_{a \samp X} [ \langle f(a, b') , \theta \rangle ] \\
     \langle X^T M_b, \theta \rangle &\geq   \langle X^T M_{b'}, \theta \rangle  \\
      X^T M_b\theta &\geq   X^T M_{b'} \theta \\
       (X^T M_b - X^T M_{b'}) \theta &\geq 0
\end{align}

The high-level idea of our algorithm is as follows. We maintain a \emph{version space} $V \subset \R^p$ of the possibilities of $\theta^*$ given the set of previous plays $(X_i, b_i)$. Specifically, the version space is the convex region
\begin{equation}
    V = \{\theta \in \R^p \mid ||\theta|| = 1 \land \forall i,b' \ X_i^T (M_{b_i} - M_{b'}) \theta  \geq 0 \}.
\end{equation}
At each stage of the game, we optimistically solve for the optimal mixed policy $X \in \Delta(A)$ such that $\theta \in V$. The chosen $X$ and $\theta$ will predict that the follower responds to $X$ with action $b'$. Let $b$ be the actual response of the follower. If $b'=b$, then $X$ was the optimal policy to play since $\theta^* \in V$ and thus one of the possible choices for $\theta$. If instead we make a \emph{mistake} and $b' \neq b$, then we receive an arbitrary loss. However, the resulting sample $(X,b)$ shrinks the version space $V$ by adding new hyperplane constraints. Next we show how to select $X$ so that when we make a mistake, $V$ is shrunk by at least some fixed volume. Since the initial volume of $V$ is finite, this will bound the number of mistakes. This procedure corresponds with linearly shrinking $V$.

Instead of naively optimizing $X \in \Delta(A)$ at each stage of the game, we solve the conservative optimization problem
\begin{equation}
    \begin{array}{ll@{}ll}
        \displaystyle\max\limits_{X \in \Delta(A)} & \displaystyle\E\limits_{a \samp X}
        \left[r^0(s,a,b_j)] \right] 
        + \E_{a \samp X} \E_{s' \samp T(s,a,b_j)} V(s')        &\\
        \text{s.t.} & X^T (M_b - M_{b'}) \theta\geq \epsilon & \forall b' \in B \\
        & \theta \in V
    \end{array}
    \label{opt:error_bound}
\end{equation}
for a fixed $\epsilon > 0$.

\begin{lemma}
If the solution $(X, \theta)$ makes a mistake in the sense that action $b$ is predicted but $b^*$ is actually played, then $V$ is shrunk by at least $V \cap B_{\frac{\epsilon}{c}}(\theta)$ where $c$ is the operator norm of $M_b - M_{b^*}$.
\end{lemma}
\begin{proof}
    From the optimization problem, we see that
    $X^T(M_b - M_{b^*}) \theta \geq \epsilon$.
    Since $b^*$ was the optimal choice for the follower agent, we have $X^T(M_{b^*} - M_b) \theta \geq 0$. Putting these together, we have
    \begin{align*}
        X^T(M_b - M_{b^*}) \theta - X^T(M_b - M_{b^*}) \theta^* &\geq \epsilon \\
        X^T (M_b - M_{b^*}) (\theta - \theta^*) &\geq \epsilon \\
        ||X^T (M_b - M_{b^*})|| \cdot ||\theta - \theta^*|| &\geq \epsilon \\
        ||X^T|| c \cdot ||\theta - \theta^*|| &\geq \epsilon \\
        ||\theta - \theta^*|| &\geq \frac{\epsilon}{c} 
    \end{align*}
Therefore $\theta^* \not\in B_{\frac{\epsilon}{c}}(\theta)$.
\end{proof}

\begin{lemma}
Using the above procedure, solutions $(X,\theta)$ to the above optimization problem produce mistakes at most $O((\frac{1}{\epsilon})^{p-1})$ times. 
\end{lemma}
\begin{proof}
Let $c$ be the max operator norm of all matrices $M_b - M_{b'}$ for $b,b' \in B$.
Since we shrink $V$ by at least $V \cap B_{\frac{\epsilon}{c}}(\theta)$ with each mistake, the number of mistakes is upper-bounded by the number of $\frac{\epsilon}{c}$-balls that can fit in the initial space $V_0 = \{\theta \in R^p \mid ||\theta|| = 1\}$.
\end{proof}

We know that whenever the solution $(X, \theta)$ results in a mistake, we incur arbitrary loss. However, as we showed, this occurs a bounded number of times. The next logical question to ask is, whenever the solution $(X, \theta)$ does not make a mistake, how much loss does it incur? Since $w^* \in V$ at all times, the solution is at least as good as the case in which $w = w^*$. So, we can just consider the case in which we solve with $w=w^*$ and we know that we do at least that well. Hence, the suboptimality of our solution is bounded by the difference between the solution to 
\begin{equation}
    \begin{array}{ll@{}ll}
        \displaystyle\max\limits_{X \in \Delta(A)} & \displaystyle\E\limits_{a \samp X}
        \left[r^0(s,a,b_j)] \right] 
        + \E_{a \samp X} \E_{s' \samp T(s,a,b_j)} V(s')        &\\
        \text{s.t.} & X^T (M_b - M_{b'}) \theta^* \geq \epsilon & \forall b' \in B \\
    \end{array}
    \label{opt:epsilon_bound}
\end{equation}
and to
\begin{equation}
    \begin{array}{ll@{}ll}
        \displaystyle\max\limits_{X \in \Delta(A)} & \displaystyle\E\limits_{a \samp X}
        \left[r^0(s,a,b_j)] \right] 
        + \E_{a \samp X} \E_{s' \samp T(s,a,b_j)} V(s')        &\\
        \text{s.t.} & X^T (M_b - M_{b'}) \theta^* \geq 0 & \forall b' \in B \\
    \end{array}
    \label{opt:zero_bound}
\end{equation}

% Let $X^*$ represent the optimal solution to (\ref{opt:zero_bound}). There exists a feasible solution $X_{b,b'}$ to (\ref{opt:zero_bound}) such that $X^T(M_b - M_{b'})$ corresponds to perturbing ${X^*}^T(M_b - M_{b'})$ in the direction $\theta^*$ by $\epsilon$ \fromnik{The previous sentence is only true under the assumption that $M_b - M_{b'}$ is full rank which in turn requires $p \leq n$}. $X_{b,b'}$ isn't necessarily a feasible solution to (\ref{opt:epsilon_bound}).

The difference in optimality between the solution (\ref{opt:zero_bound}) and to (\ref{opt:error_bound}) is bounded by the maximum difference in optimality induced by two solutions that differ by the Hausdorff distance between the feasibility regions. The Hausdorff distance is realized at the critical points of the feasibility region of (\ref{opt:zero_bound}). Let $C \subset B$, $|C| = q$ represent a critical boundary of the feasibility space of (\ref{opt:zero_bound}). That is, there exists some ${X^*}^T$ such that ${X^*}^T (M_b - M_{b'}) \theta^* = 0$ for all $b' \in C$. 

Therefore, the Hausdorff distance is upperbounded by the maximum distance between $X^*$ subject to ${X^*}^T (M_b - M_{b'}) \theta^* = 0$ and 
$X$ subject to ${X}^T (M_b - M_{b'}) \theta^* = \epsilon$ for all $b' \in C$ over all $C \subset B$.
So we have $({X}^T - {X^*}^T)(M_b - M_{b'}) \theta^* = 0$ for all $b' \in C$.

Define a projection matrix $M \in \R^{n \times q}$ such that $[M]^{b'} = (M_b - M_{b'}) \theta^*$. Then we have
\begin{equation}
    (X^T - {X^*}^T) M = \bar{\epsilon}
\end{equation}
where $\bar{\epsilon} = (\epsilon, \dots, \epsilon)$. 
If $q \geq n$, then $M$ is a right inverse. Rearranging, this gives 
\begin{align}
    ||(X^T - {X^*}^T)|| &= ||\bar{\epsilon} M^{\dagger} ||\\
    &\leq \sqrt{q} \cdot \epsilon \cdot d \\
    &\leq \sqrt{m} \cdot \epsilon \cdot d
\end{align}
 since $m \leq q$ where $d$ is the operator norm of $M^{\dagger}$. 

If instead $q < n$, then we make use of the following lemma (with proof left to the appendix).

\begin{lemma}
Let $M \in \R^{n \times q}$ with $q < n$ with rank $q$. If $X^T M = \bar{\epsilon}$, then there exists a full rank matrix $M' \in \R^{n \times n}$ with the first $q$ columns identical to $M$ such that $X^T M' = (\bar{\epsilon}, \bar{0})$. Moreover, $M'$ can be constructed to have minimum singular value equal to the minimum singular value of $M$. 
\end{lemma}

Therefore we have that
\begin{align}
    ||(X^T - {X^*}^T)|| &= ||(\bar{\epsilon}, \bar{0}) M'^{-1} ||\\
    &\leq \sqrt{q} \cdot \epsilon \cdot d \\
    &\leq \sqrt{m} \cdot \epsilon \cdot d
\end{align}
where $d = \opnorm{M'^{-1}}$. 

This result gives the following lemma.

% The difference in value between the two optimization problems is upperbounded by the difference in value of the Hausdorff distance between the two feasibility regions. In fact, since the optimization problem is linear, the solution $X^*$ to (\ref{opt:zero_bound}) and $X$ to (\ref{opt:error_bound}) satisfies
% \begin{equation}
%     ||X^T(M_b - M_{b'}) - {X^*}^T(M_b - M_{b'})|| \leq \epsilon
% \end{equation}
% for all $b,b' \in B$. \fromnik{I'm not 100\% sure about this claim. Needs to be more convincing.} Therefore, we have that $||X^T - {X^*}^T|| \leq \frac{\epsilon}{c}$ which in turn bounds
% \begin{align}
%     \E\limits_{a \samp X} \left[r^0(s,a,b_j)] \right] - \E\limits_{a \samp X^*} \left[r^0(s,a,b_j)] \right]& \\
%      = (X^T  - {X^*}^T) R^0_{s,b} &\leq ||X^T - {X^*}^T|| \cdot ||R^0_{s,b}|| \\
%      &\leq \frac{\epsilon}{c} \cdot ||R^0_{s,b}|| \\
%      &\leq \frac{\epsilon}{c} \cdot \sqrt{n}
% \end{align}
% since $R^0_{s,b} \in [0,1]^n$. \fromnik{ Note that this analysis ignores the the future states and therefore the future discounted reward. I think a similar analysis should bound the difference in reward while taking future states into account.}

\begin{lemma}
If a solution $(X,\theta)$ to the above optimization problem does not make a mistake, then it incurs regret at most $\epsilon \cdot d \cdot \sqrt{mn}$ where $d$ is the operator norm of $M^{-1}$ as constructed above.
\end{lemma}
\begin{proof}
 We have that $||X^T - {X^*}^T|| \leq \sqrt{m} \cdot \epsilon \cdot d$ from above which in turn bounds,
\begin{align}
    \E\limits_{a \samp X} \left[r^0(s,a,b_j)] \right] - \E\limits_{a \samp X^*} \left[r^0(s,a,b_j)] \right]& \\
     = (X^T  - {X^*}^T) R^0_{s,b} &\leq ||X^T - {X^*}^T|| \cdot ||R^0_{s,b}|| \\
     &\leq \epsilon \cdot d \cdot \sqrt{m} \cdot ||R^0_{s,b}|| \\
     &\leq \epsilon \cdot d \cdot \sqrt{m} \cdot \sqrt{n}
\end{align}
since $R^0_{s,b} \in [0,1]^n$. \fromnik{ Note that this analysis ignores the the future states and therefore the future discounted reward. I think a similar analysis should bound the difference in reward while taking future states into account.}
\end{proof}

The \emph{local regret} against policy $\pi^*$ that chooses mixed policies $X^*$ is
\begin{equation}
    R_{h,T}(s) = \E \left[ \sum_{t=1}^T \left( \E_{a \samp {X_t^*}}[Q_{t,h}(s,a)] - \E_{a \samp X_t} \left[Q_{t,h} (s,a) \right] \right) \right] 
\end{equation}
Since $R_{T,h} = \E_{S^*_h \samp \mu^*_h}[R_{h,T}(S^*_h)]$, we have $R_T = \sum_{h=1}^H R_{T,h}$. 
Therefore, the global regret is bounded by
\begin{align}
    R_T &\leq H\left(\frac{1}{\epsilon}\right)^{p-1} +  \left( \epsilon \cdot d \cdot \sqrt{mn} \right) \left(T-\left(\frac{1}{\epsilon}\right)^{p-1}\right) \label{eq:global_regret_complex_bound} \\
    &\leq H\left(\frac{1}{\epsilon}\right)^{p-1} + \left( \epsilon \cdot d \cdot \sqrt{mn} \right) T \label{eq:global_regret_simple_bound}.
\end{align}
\fromnik{Note that we lose some optimality by simplifying to (\ref{eq:global_regret_simple_bound}). How much better can we do if we optimize (\ref{eq:global_regret_complex_bound}) instead?}
Choosing $\epsilon = T^{-\frac{1}{p}}$ gives
\begin{align}
    R_T &\leq H\left(T\right)^{\frac{p-1}{p}} +  d \cdot \sqrt{mn} \cdot \left(T\right)^{\frac{p-1}{p}} \\
     &\leq \left(T\right)^{\frac{p-1}{p}} \left(H + d \cdot \sqrt{mn}\right)
\end{align}
So $R_T = O(T^{\frac{p-1}{p}})$ which is sublinear for any $p$.
